Toward Optimized VR/AR Ergonomics: Modeling and Predicting User Neck Muscle Contraction

Ergonomic efficiency is essential to the mass and prolonged adoption of VR/AR experiences. While VR/AR head-mounted displays unlock users' natural wide-range head movements during viewing, their neck muscle comfort is inevitably compromised by the added hardware weight. Unfortunately, little quantitative knowledge for understanding and addressing such an issue is available so far. Leveraging electromyography devices, we measure, model, and predict VR users' neck muscle contraction levels (MCL) while they move their heads to interact with the virtual environment. Specifically, by learning from collected physiological data, we develop a bio-physically inspired computational model to predict neck MCL under diverse head kinematic states. Beyond quantifying the cumulative MCL of completed head movements, our model can also predict potential MCL requirements with target head poses only. A series of objective evaluations and user studies demonstrate its prediction accuracy and generality, as well as its ability in reducing users' neck discomfort by optimizing the layout of visual targets. We hope this research will motivate new ergonomic-centered designs for VR/AR and interactive graphics applications. Source code is released at: https://github.com/NYU-ICL/xr-ergonomics-neck-comfort.

==> figure_captions/supplementary_emg_processing.tex <==
\begin{figure}[h!]
\begin{tcolorbox}[
    enhanced,
    attach boxed title to top left={xshift=6mm,yshift=-3mm},
    colback=moonstoneblue!20,
    colframe=moonstoneblue,
    colbacktitle=moonstoneblue,
    title=EMG to \activationShort Data Processing Pipeline,
    fonttitle=\bfseries\color{black},
    boxed title style={size=small,colframe=moonstoneblue},
    sharp corners]
\medskip
\begin{algorithmic}[1]
    \Function{EMG2\activationShort}{EMG}
        \State {\color{blue}\(\triangleright\) 4-channel EMG signals}
        \State $t = \Call{GetTimestamps}{\textsc{EMG}}$ {\color{blue} \Comment{EMG timestamps}}
        \State $\textsc{axis} = $ 0
        \State $\textsc{bandpass\_freq\_low} = $ 20 Hz
        \State $\textsc{bandpass\_freq\_high} = $ 150 Hz
        \State $\textsc{lowpass\_freq} = $ 1 Hz
        \State $\textsc{butterworth\_order} = $ 4
        \State {\color{blue}\(\triangleright\) Constant detrending}
        \State $\textsc{EMG} = \textsc{EMG} - \Call{Mean}{\textsc{EMG}, \textsc{axis}}$
        \State {\color{blue}\(\triangleright\) 4th order Butterworth bandpass filter}
        \State $\textsc{sampling\_rate} = \Call{Len}{\textsc{EMG}} / (t[-1] - t[0])$
        \State $\textsc{low} = $ $(2 * \textsc{bandpass\_freq\_low}) / \textsc{sampling\_rate}$
        \State $\textsc{high} = $ $(2 * \textsc{bandpass\_freq\_high}) / \textsc{sampling\_rate}$
        \State $\textsc{EMG} = \Call{sos\_bp}{\textsc{EMG}, \textsc{order}, [\textsc{low}, \textsc{high}], \textsc{axis}}$
        \State {\color{blue}\(\triangleright\) RMS envelope filter}
        \State $\textsc{window} = $  [1/1000, ..., 1/1000] {\color{blue} \Comment{1000-length}}
        \State {\textbf{for} i $\gets$ $[0,4)$ \textbf{do}:}
            \State \hskip1em $\textsc{EMG[$i$]} = \sqrt{\Call{conv}{\textsc{EMG[$i$]}^2, \textsc{window}}}$
        \State {\color{blue}\(\triangleright\) 4th order Butterworth lowpass filter}
        \State $\textsc{low} = $ $(2 * \textsc{lowpass\_freq}) / \textsc{sampling\_rate}$
        \State $\textsc{EMG} = $ \Call{sos\_lp}{\textsc{EMG}, \textsc{order}, \textsc{low}, \textsc{axis}}
        \State {\color{blue}\(\triangleright\) Left/Right normalization}
        \State $\textsc{EMG[0]} = \Call{max}{\textsc{EMG[1]}}/\Call{max}{\textsc{EMG[0]}}$ 
        \State $\textsc{EMG[2]} = \Call{max}{\textsc{EMG[3]}}/\Call{max}{\textsc{EMG[2]}}$ 
        \State {\color{blue}\(\triangleright\) Compute overall \activationShort}
        \State $\textsc{axis} = $ 1
        \State \textbf{return} $\Call{sum}{\textsc{EMG}, \textsc{axis}}$ {\color{blue} \Comment{Channel-wise sum}}
    \EndFunction
\end{algorithmic}
\end{tcolorbox}
\Caption{Our EMG data processing pipeline.}{The illustrated function filters and transforms multi-channel raw EMG signals into overall neck \activationShort.}
\label{fig:emg-processing-pseudo-code}
\end{figure}

==> figure_captions/supplementary_user_study_conditions.tex <==
\begin{figure}[ht]
\begin{tcolorbox}[
    enhanced,
    attach boxed title to top left={xshift=6mm,yshift=-3mm},
    colback=moonstoneblue!20,
    colframe=moonstoneblue,
    colbacktitle=moonstoneblue,
    title=User Study Condition Generation,
    fonttitle=\bfseries\color{black},
    boxed title style={size=small,colframe=moonstoneblue},
    sharp corners]
\medskip
\begin{algorithmic}[1]
    \Function{GetNextPose}{$\RotationStart$, $\TimeStamp$, $\theta^\circ$, \textsc{Condition}}
        \State {\color{blue}\(\triangleright\) Unif. sample 180 head poses that are $\theta^\circ$ from $\RotationStart$}
        \State $\textsc{poses} = \Call{UniformSample}{\RotationStart, \theta^\circ, 180}$
        \State $\textsc{all\_traj} = []$ 
        \State {\textbf{for} $\RotationEnd$ $\gets$ \textsc{poses} \textbf{do}:}
            \State \hskip1em {\color{blue}\(\triangleright\) Predict the head trajectory from $\RotationStart$ to $\RotationEnd$}
            \State \hskip1em $\textsc{trajectory} = \Call{\TrajectoryNet}{\RotationStart,\RotationEnd}$
            \State \hskip1em {\color{blue}\(\triangleright\) Include 1-second fixation on $\RotationEnd$}
            \State \hskip1em $\textsc{trajectory} = \Call{AddFixation}{\textsc{trajectory},\RotationEnd}$
            \State \hskip1em \textsc{all\_traj}.\Call{Append}{\textsc{trajectory}}
        \State {\color{blue}\(\triangleright\) Pick candidate with highest score as next pose}
        \State $\textsc{maxScore} = -\textsc{Inf}$
        \State \textsc{Init} $\PilotTargetPos$ {\color{blue} \Comment{Current candidate for next pose}}
        \State {\textbf{for} $i$ $\gets$ [0, ..., \Call{len}{\textsc{all\_traj}}-1] \textbf{do}:}
            \State \hskip1em $\RotationEnd = \Call{GetEndPose}{\textsc{all\_traj}[i]}$
            \State \hskip1em {\textbf{if} \textsc{Condition} == $\conditionMax$:}
                \State \hskip2em $\textsc{score} = \CoverageEnergy(\PilotTargetPos_{j\in[1,\TimeStamp]},\RotationEnd)+\CombinedEnergy(\textsc{all\_traj}[i])$
            \State \hskip1em {\textbf{if} \textsc{Condition} == $\conditionRand$:}
                \State \hskip2em $\textsc{score} = \CoverageEnergy(\PilotTargetPos_{j\in[1,\TimeStamp]},\RotationEnd)$
            \State \hskip1em {\textbf{if} \textsc{Condition} == $\conditionMin$:}
                \State \hskip2em $\textsc{score} = \CoverageEnergy(\PilotTargetPos_{j\in[1,\TimeStamp]},\RotationEnd)-\CombinedEnergy(\textsc{all\_traj}[i])$ 
            \State \hskip1em {\color{blue}\(\triangleright\) Update $\PilotTargetPos$ if $\textsc{score}$ greater than $\textsc{maxScore}$}
            \State \hskip1em {\textbf{if} $\textsc{score} > \textsc{maxScore}$:}
                \State \hskip2em $\textsc{maxScore} = \textsc{Score}$
                \State \hskip2em $\PilotTargetPos = \RotationEnd$
        \State \textbf{return} $\PilotTargetPos$
    \EndFunction
\end{algorithmic}
\end{tcolorbox}
\Caption{User study condition generation algorithm.}{Given the current head pose $\RotationEnd$ on a scan path, this function extends the scan path by generating the optimal next head pose $\PilotTargetPos$ for one of the 3 conditions $\conditionMax$/$\conditionMin$/$\conditionRand$.}
\label{fig:user-study-conditions-pseudo-code}
\end{figure}

==> figure_captions/tab_user_study.tex <==
\begin{table}[!hbp]
\begin{adjustbox}{max width=0.48\textwidth}
  \centering
  \tabtextsize
  \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \diagbox{cond}{user} & \#1 & \#2 & \#3 & \#4 & \#5 & \#6 & \#7 & \#8 & \#9 & \#10 & \#11 & \#12\\
    \hline
    $\conditionMax$& 11 & 12 & 11 & 12 & 10 & 10 & 9 & 12 & 9 & 10 & 9 & 9\\
    \hline
    $\conditionRand$& 5 & 5 & 6 & 4 & 4 & 7 & 8 & 6 & 7 & 6 & 6 & 9\\
    \hline
    $\conditionMin$& 2 & 1 & 1 & 2 & 4 & 1 & 1 & 0 & 2 & 2 & 3 & 0\\
    \hline
  \end{tabular}
  \end{adjustbox}
  \Caption{Individual 2AFC results in user study.}{The numbers indicate, for each participant and each condition, how many trials among all 18 2AFC sessions that particular condition was rated by that particular participant as being more uncomfortable.}
  \label{tab:user-study}
\end{table}

==> tools/hackstyle.tex <==
\setlength{\abovecaptionskip}{1.0ex}
\setlength{\belowcaptionskip}{1.0ex}
\setlength{\floatsep}{1.0ex}
\setlength{\dblfloatsep}{\floatsep}
\setlength{\textfloatsep}{2.0ex}
\setlength{\dbltextfloatsep}{\textfloatsep}
\setlength{\abovedisplayskip}{1.0ex}
\setlength{\belowdisplayskip}{1.0ex}
